Perfectly Parallel Fairness Certification of Neural Networks

Recently, there is growing concern that machine-learning models, which currently assist or even automate decision making, reproduce, and in the worst case reinforce, bias of the training data. The development of tools and techniques for certifying fairness of these models or describing their biased behavior is, therefore, critical. In this paper, we propose a perfectly parallel static analysis for certifying causal fairness of feed-forward neural networks used for classification of tabular data. When certification succeeds, our approach provides definite guarantees, otherwise, it describes and quantifies the biased behavior. We design the analysis to be sound, in practice also exact, and configurable in terms of scalability and precision, thereby enabling pay-as-you-go certification. We implement our approach in an open-source tool and demonstrate its effectiveness on models trained with popular datasets.

==> censusT.tex <==
%!TEX root = paper.tex
\centering
\resizebox{0.75\textwidth}{!}{%
\begin{tabular}{|c|c|cc|cc|cc|}
\hline
\multirow{2}{*}{$\size{\model}$} & 
\multirow{2}{*}{$\upperbound$} & 
\multicolumn{2}{c|}{\textsc{boxes}} & 
\multicolumn{2}{c|}{\textsc{boxes+symbolic}} &
\multicolumn{2}{c|}{\textsc{deeppoly}} \\
& & 
\textsc{input} & \textsc{time} &
\textsc{input} & \textsc{time} &
\textsc{input} & \textsc{time} \\
\hline%
\rowcolor{gray!10}
\cellcolor{mygreen!30} & $4$ 
& {\small $86.81\%$} &  {\small 28m 2s} 
& {\small $93.61\%$} &  {\small 16m 57s} 
& {\small $93.13\%$} &  {\small 1h 9m 26s} \\
%\rowcolor{mygreen!30}
\cellcolor{mygreen!30} & $6$ 
& {\small $99.51\%$} & {\small 59m 15s} 
& {\small $99.93\%$} & {\small 39m 16s} 
& {\small $99.83\%$} &  {\small 1h 35m 42s} \\
\rowcolor{gray!10}
\cellcolor{mygreen!30} & $8$ 
& {\small $100.00\%$} & {\small 4h 55m 57s} 
& {\small $100.00\%$} &  {\small 3h 24m 42s} 
& {\small $100.00\%$} &  {\small 6h 58m 17s} \\
%\rowcolor{mygreen!30}
\multirow{-4}{*}{\cellcolor{mygreen!30}\begin{tabular}{c}$10$\\$\showmark{o}\showmark{*}\showmark{oplus}$\end{tabular}}
 & $10$ 
& {\small $100.00\%$} & {\small 56m 18s} 
& {\small $100.00\%$} & {\small 56m 22s} 
& {\small $100.00\%$} &  {\small 56m 37s} \\
\hline%%%%%%%%%
\rowcolor{gray!10}
\cellcolor{myyellow!30} & $4$ 
& {\small $49.76\%$} &  {\small 12m 26s} 
& {\small $72.22\%$} &  {\small 21m 48s} 
& {\small $60.59\%$} &  {\small 10m 0s} \\
%\rowcolor{myyellow!30}
\cellcolor{myyellow!30} & $6$ 
& {\small $72.67\%$} & {\small 2h 2m 57s} 
& {\small $98.54\%$} & {\small 20m 38s} 
& {\small $66.35\%$} &  {\small 15m 55s} \\
\rowcolor{gray!10}
\cellcolor{myyellow!30} & $8$ 
& {\small $98.68\%$} & {\small 1h 38m 31s} 
& {\small $98.78\%$} &  {\small 41m 0s} 
& {\small $70.87\%$} &  {\small 2h 17m 47s} \\
%\rowcolor{myyellow!30}
\multirow{-4}{*}{\cellcolor{myyellow!30}\begin{tabular}{c}$12$\\$\showmark{triangle}\showmark{triangle*}\showmark{Mercedes
 star}$\end{tabular}}
 & $10$ 
& {\small $99.06\%$} & {\small 1h 25m 42s} 
& {\small $99.06\%$} & {\small 1h 12m 5s} 
& {\small $80.76\%$} &  {\small 2h 53m 32s} \\
\hline%%%%%%%%%
\rowcolor{gray!10}
\cellcolor{myorange!30} & $4$ 
& {\small $22.01\%$} & {\small \small  2m 6s}
& {\small $44.06\%$} & {\small \small  14m 26s} 
& {\small $42.08\%$} &  {\small 2m 48s} \\
%\rowcolor{myorange!30}
\cellcolor{myorange!30} & $6$ 
& {\small $45.24\%$} & {\small \small  21m 30s}
& {\small $60.03\%$} & {\small \small  42m 22s} 
& {\small $58.61\%$} &  {\small 21m 39s} \\
\rowcolor{gray!10}
\cellcolor{myorange!30} & $8$ 
& {\small $64.17\%$} & {\small 2h 46m 48s}
& {\small $74.10\%$} & {\small 2h 8m 25s} 
& {\small $69.72\%$} &  {\small 2h 3m 3s} \\
%\rowcolor{myorange!30}
\multirow{-4}{*}{\cellcolor{myorange!30}\begin{tabular}{c}$20$\\$\showmark{diamond}\showmark{diamond*}\testmark{myorange!30}{halfdiamond*}$\end{tabular}}
 & $10$ 
& {\small $85.87\%$} & {\small >13h}
& {\small $89.24\%$} & {\small >13h} 
& {\small $76.18\%$} &  {\small 5h 5m 2s} \\
\hline%%%%%%%%%
\rowcolor{gray!10}
\cellcolor{myred!30} & $4$ 
& {\small $0.00\%	$} & {\small  1m 5s      }
& {\small $0.69\%	$} & {\small  3m 33s     } 
& {\small $0.80\%$} &  {\small 8m 52s} \\
%\rowcolor{myred!30}
\cellcolor{myred!30} & $6$ 
& {\small $0.00\%	$} & {\small  1m 5s      }
& {\small $3.19\%	$} & {\small  40m 40s    } 
& {\small $2.99\%$} &  {\small 1h 21m 45s} \\
\rowcolor{gray!10}
\cellcolor{myred!30} & $8$ 
& {\small $0.14\%	$} & {\small  13m 58s    }
& {\small $9.48\%	$} & {\small 2h 40m 43s    } 
& {\small $8.54\%$} &  {\small 2h 38m 13s} \\
%\rowcolor{myred!30}
\multirow{-4}{*}{\cellcolor{myred!30}\begin{tabular}{c}$40$\\$\showmark{square}\showmark{square*}\testmark{myred!30}{halfsquare*}$\end{tabular}}
 & $10$ 
& {\small $0.63\%	$} & {\small 1h 48m 43s    }
& {\small $19.62\%	$} & {\small 12h 25m 43s} 
& {\small $19.41\%$} &  {\small >13h} \\
\hline%%%%%%%%%
\rowcolor{gray!10}
\cellcolor{mypurple!30} & $4$ 
& {\small $0.00\%	$} & {\small  1m 9s  }
& {\small $27.26\%	$} & {\small  8m 24s } 
& {\small $11.42\%$} &  {\small 1m 54s} \\
%\rowcolor{mypurple!30}
\cellcolor{mypurple!30} & $6$ 
& {\small $0.83\%	$} & {\small  3m 44s }
& {\small $39.65\%	$} & {\small  24m 1s } 
& {\small $27.47\%$} &  {\small 4m 25s} \\
\rowcolor{gray!10}
\cellcolor{mypurple!30} & $8$ 
& {\small $9.41\%	$} & {\small  22m 49s}
& {\small $47.47\%	$} & {\small  55m 30s} 
& {\small $37.36\%$} &  {\small 29m 56s} \\
%\rowcolor{mypurple!30}
\multirow{-4}{*}{\cellcolor{mypurple!30}\begin{tabular}{c}$45$\\$\showmark{pentagon}\showmark{pentagon*}\showmark{10-pointed
 star}$\end{tabular}}
 & $10$ 
& {\small $18.68\%	$} & {\small 1h 39m 33s}
& {\small $49.62\%	$} & {\small 3h 24m 15s} 
& {\small $46.39\%$} &  {\small 2h 13m 49s} \\
%
\hline
\end{tabular}
}
